NLU++: A Multi-Label, Slot-Rich, Generalisable Dataset for Natural Language Understanding in Task-Oriented Dialogue

We present NLU++, a novel dataset for natural language understanding (NLU) in task-oriented dialogue (ToD) systems, with the aim to provide a much more challenging evaluation environment for dialogue NLU models, up to date with the current application and industry requirements. NLU++ is divided into two domains (BANKING and HOTELS) and brings several crucial improvements over current commonly used NLU datasets. 1) NLU++ provides fine-grained domain ontologies with a large set of challenging multi-intent sentences, introducing and validating the idea of intent modules that can be combined into complex intents that convey complex user goals, combined with finer-grained and thus more challenging slot sets. 2) The ontology is divided into domain-specific and generic (i.e., domain-universal) intent modules that overlap across domains, promoting cross-domain reusability of annotated examples. 3) The dataset design has been inspired by the problems observed in industrial ToD systems, and 4) it has been collected, filtered and carefully annotated by dialogue NLU experts, yielding high-quality annotated data. Finally, we benchmark a series of current state-of-the-art NLU models on NLU++; the results demonstrate the challenging nature of the dataset, especially in low-data regimes, the validity of `intent modularisation', and call for further research on ToD NLU.

==> 06_discussion.tex <==



\section{Discussion}

\subsection{Generic ontology definition}

While we are not claiming that this is the \textit{definitive} generic ontology and that every dataset should follow it, this proves that a more \textit{intelligent} design of the ontologies could massively help with data reusability on NLU. However, the definition of these intents is not trivial, and sometimes the boundaries of the generic intents are not clear at all, even for expert annotators. Some intents like \textit{greet}, \textit{why} and \textit{change} are quite clear, while for others such as \textit{make} or \textit{not\_working} boundaries are not so clear. Slots like \textit{time} and \textit{date} are very clear.

\subsection{Span based VE}\label{VE_discussion}
As mentioned in section \ref{sec:slots}, span-based annotation, training and evaluation can be suboptimal. For example, in the sentence \textit{Book it for the 7th of June} the minimal annotated span should be \textit{7th of June}. However, if \textit{the 7th of June} is detected as the span, the evaluation will detect it as an error. However, any value parser would correctly parse both sentences. In addition, a slot-filling model trained on minimal span annotations will lean towards dropping information (e.g. for the \textit{time} slot, we have observed that several errors are caused by the span not including the AM/PM part of the time). Annotators are also more prone to make mistakes when annotating spans in this style, and these discrepancies will reflect in a loss of performance in the evaluation. Finally, separating intervals as \textit{date\_from} and \textit{date\_to} or even times and dates also increases the complexity of the task. Times and dates could be annotated together, and more complex parsers be used to get the values, moving complexity from the annotation and slot filling models to the parsers.

\subsection{Contextual utterances}
While NLU has pivoted from full dialogue history DST to single user utterance classification, some user utterances only make sense on the context of the previous system utterance. For example, the answer \textit{4}, might refer to a date, a number of people, an amount of money... depending on the previous system question. In the case of dates, \textit{July 4th} could be \textit{date\_from} or \textit{date\_to} depending on the previous context. In the same way it could be argued that some intents like \textit{affirm} and \textit{deny} only make sense in the context of the previous system question. \cite{CoopeFarghly2020} proposed using discrete annotations in order to indicate if a specific slot had been requested by the system. However this creates an extra annotation requirement as well as a extra learning requirement for the model. In this work, we propose using \textit{uncontextualised} slots such as \textit{number}, \textit{time} and \textit{date} to extract those values, while letting the policy to contextualise them if necessary. This reduces annotation efforts and the learning requirements of the model, while not requiring any extra information since the policy would have to pass the \textit{requested slot} to the NLU model anyway.

However, we think that as NLU models become more and more data efficient, NLU datasets should start evolving towards \textit{system turn + user turn} datasets, so that the contextual nature of these queries can be solved in a more natural way.

\subsection{Intent and slot relations}

When pivoting towards heavy multi-intent ontologies, a sentence to intents mapping might not be enough anymore. For example, in the sentence, \textit{can you add one more kid to my 4 adults reservation?}, the intent \textit{more} is related to the slot \textit{kids}, not to the slot \textit{adults}. In a more extreme case, the sentences \textit{no, cancel it} and \textit{don't cancel it} could be both labelled as \textit{deny, cancel}, while they mean the opposite. Some research on this topic has already been done in the ATIS dataset \cite{gangadharaiah-narayanaswamy-2019-joint}. While out of the scope of this work, we think that future NLU datasets should take this into account.
